Neural Enhanced Belief Propagation for Multiobject Tracking

Algorithmic solutions for multi-object tracking (MOT) are a key enabler for applications in autonomous navigation and applied ocean sciences. State-of-the-art MOT methods fully rely on a statistical model and typically use preprocessed sensor data as measurements. In particular, measurements are produced by a detector that extracts potential object locations from the raw sensor data collected for a discrete time step. This preparatory processing step reduces data flow and computational complexity but may result in a loss of information. State-of-the-art Bayesian MOT methods that are based on belief propagation (BP) systematically exploit graph structures of the statistical model to reduce computational complexity and improve scalability. However, as a fully model-based approach, BP can only provide suboptimal estimates when there is a mismatch between the statistical model and the true data-generating process. Existing BP-based MOT methods can further only make use of preprocessed measurements. In this paper, we introduce a variant of BP that combines model-based with data-driven MOT. The proposed neural enhanced belief propagation (NEBP) method complements the statistical model of BP by information learned from raw sensor data. This approach conjectures that the learned information can reduce model mismatch and thus improve data association and false alarm rejection. Our NEBP method improves tracking performance compared to model-based methods. At the same time, it inherits the advantages of BP-based MOT, i.e., it scales only quadratically in the number of objects, and it can thus generate and maintain a large number of object tracks. We evaluate the performance of our NEBP approach for MOT on the nuScenes autonomous driving dataset and demonstrate that it has state-of-the-art performance.

==> LatexInclusion/catechism.tex <==
%----------------------------------------------------------------------------------------%
%                                       C a t e c h i s m                                         %
%----------------------------------------------------------------------------------------%
\section*{Research Paper Catechism\footnote{Adapted from George Heilmeier.}} 

\vspace{0.5cm} 

\be\itemsep3ex

\item What is the big picture? What is the problem and why is it hard?
	\bi
	\item[$\diamond$] The Big Picture: \BigPicture
	\item[$\diamond$] The Problem/Difficulty: \ProblemDifficulty
%	\item[$\diamond$] The Difficulty:
	\ei

\item What are the classical approaches? What is the state-of-the-art and what are the deficiencies?
	\bi
	\item[$\diamond$] Classical Approaches: \ClassicApproach
	\item[$\diamond$] The State-of-the-Art and Deficiencies:  \SOADeficiency
	\item[ ] \mysubsubnote{This is where you make a literature review. Articulate the deficiencies and shortcomings of previous work. Provide references (you can use the first three alphabets of the authors' last names and year, similar to the convention in our database).}
	\ei
	
\item What are the fundamental questions relevant to the problem? How answering to these questions can impact the design, architecture, and operation?
	\bi
	\item[$\circ$] \FundamentalQ
	\item[$\circ$] \EnablingA 
	\item[ ] \mysubsubnote{This is where you persuade the reader that these are fundamental questions, and the answers to these questions will have game-changing impacts.}
	\ei	

\item What are the goals of our paper?
	\bi
	\item[$\diamond$] The Goals:
	\item[ ] \mysubsubnote{Describe the goals at a high level; this should correlate with high-level contributions in Question 6.}
	\ei
		\be
		\item[$\circ$] \Goals 
		\ee		

\item What are we advocating; what is the new technical idea; what is our new view; what is our credence? Why we can succeed now? 
	\bi
	\item[$\diamond$] Advocacy, Idea, View, and Credence:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \Advocacy 
		\ee
	\item[$\diamond$] Reasons for Success:
	\item[ ] \mysubsubnote{For example:}
		\be
		\item[$\circ$] \ReasonSuccess 
		\ee
	\ei

\item What are the high-level contributions of our  paper? What are the key contributions of our paper? 
	\bi
	\item[$\diamond$] High-Level Contributions: \HLContribution
	\item[ ] \mysubsubnote{Describe what we do at a high level; this should address the goal that we set out in Question 4; for example:}
		\be
		\item[$\circ$] In this paper, \ldots
		\ee
	\item[$\diamond$] Key Contributions:
	\item[ ] \mysubsubnote{Provide a bulletized list (usually 3-5 bullets, equal number of lines per bullets); for example:}
		\be
		\item[$\circ$] \KeyContribution
		\ee
	\ei


\item Which are the methodologies (analysis, simulation, experimentation, heterogeneous approach) used in this paper? How is the approach verified; how are the results confirmed?
	\bi
	\item[$\diamond$] The Methodologies: Belief propagation, factor graphs, graph neural networks
	\item[$\diamond$] The Verification: The proposed algorithm will be evaluated on nuScenes tracking dataset.
	\ei
	
\item What are the new vision/perspective we provide? What are the lessons learned?
	\bi
	\item[$\diamond$] The New Vision/Perspective: \ConclusiveVision
	\item[$\diamond$] The Lessons Learned/Surprising Results: \ConclusiveLesson
	\ei

\item What is the impact; what are the benefits or merits of the results to a broader community?
	\bi
	\item[$\diamond$] The Impact/Benefit: \Benefit
	\item[ ] \mysubsubnote{Think of strong conclusions for the paper when answering them}
	\ei


\item Where the known results appear in the paper?
	\bi
	\item[$\diamond$] Disclosures: Statistical modeling of the \ac{mot} problem is introduced in Section \ref{sec:model} and the \ac{bp}-based \ac{mot} algorithm is reviewed in \ref{sec:bp}.
	\item[ ] \mysubsubnote{Identify where known results appear in the paper (point to specific section numbers before the paper is written; point to specific section, page, line, equation numbers, etc. after the paper is written).}
	\item[$\diamond$] Sources: \ac{bp}-based \ac{mot} algorithm \cite{WilLau:J14,MeyBraWilHla:J17,MeyKroWilLauHlaBraWin:J18}.
	\item[ ] \mysubsubnote{Identify what are the sources (provide reference, section, page, line, equation numbers, etc. of the sources).}
	\ei

\item What are the key references?
\bi
	\item[ ] \mysubsubnote{List the key references that we used to develop this paper (rather than the references for the state-of-the-art).}
	
	\ac{bp} \cite{KscFreLoe:01,YedFreWei:05,KolFri:B09}; \acp{gnn} \cite{GorMonSca:05, GilSchRilVinDah:17}; \ac{bp} with deep learning \cite{YooLiaXioZhaFetUrtZemPit:19, KucChaTanLuoSonSabErm:20, SatWel:21}; \ac{mot} \cite{BarWilTia:B11, Mah:B07}
% 	object detectors \cite{YinZhoKra:21, ZhuJiaZhoLiYu:19, LanVorCaeZhoYanBei:19}; nuScenes dataset \cite{CaeBanLanVorLioXuKriPanBalBei:20}
	
% 	MOT (``point target''): \cite{BarWilTia:B11,Mah:B07,MeyKroWilLauHlaBraWin:J18}; EOT \cite{HabThaKirGriWak:C11,HamSveSanSor:J12,HabThaThaMalKir:J13
% 	,SchReuWan:C15,CorCar:J18,GenVivBraSolAmi:J15,VivBra:J16,GraOrg:J12,LunGraOrg:J13,BeaReuGraVoVoSch:J16,GraFatSve:J17}: 
\ei

\ee


==> LatexInclusion/defmetric.tex <==
% put your latex definitions here.
% For example: \newcommand{\samplesize}{n}

%---------------------%
% Symbols             %
%---------------------%


%---------------------%
% References        %
%---------------------%
%\newcommand{\fig}[1]{Fig.~\ref{#1}}
%\newcommand{\sect}[1]{Sec.~\ref{#1}}
%\newcommand{\apd}[1]{Appendix~\ref{#1}}
%\newcommand{\eq}[1]{(\ref{#1})}


%--------------------------------------------------------------%
% List: Using description, enumerate, itemize       %
%--------------------------------------------------------------%

\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bl}{\begin{list}}
\newcommand{\el}{\end{list}}
\newcommand{\bt}{\begin{tabbing}}
\newcommand{\et}{\end{tabbing}}

\providecommand{\cbl}{\textcolor{blue}}
\providecommand{\crd}{\textcolor{red}}

%--------------------------------------------------------------%
% Define color specifically for MarkBoth 		  %
%--------------------------------------------------------------%
\definecolor{BLUE}{rgb}{0,0,1}

